QTRAN: Learning to Factorize with Transformation for Cooperative Multi-Agent Reinforcement Learning

We explore value-based solutions for multi-agent reinforcement learning (MARL) tasks in the centralized training with decentralized execution (CTDE) regime popularized recently. However, VDN and QMIX are representative examples that use the idea of factorization of the joint action-value function into individual ones for decentralized execution. VDN and QMIX address only a fraction of factorizable MARL tasks due to their structural constraint in factorization such as additivity and monotonicity. In this paper, we propose a new factorization method for MARL, QTRAN, which is free from such structural constraints and takes on a new approach to transforming the original joint action-value function into an easily factorizable one, with the same optimal actions. QTRAN guarantees more general factorization than VDN or QMIX, thus covering a much wider class of MARL tasks than does previous methods. Our experiments for the tasks of multi-domain Gaussian-squeeze and modified predator-prey demonstrate QTRAN's superior performance with especially larger margins in games whose payoffs penalize non-cooperative behavior more aggressively.

==> 2.intro.tex <==
\section{Introduction}

Reinforcement learning aims to instill in agents a good policy that maximizes the cumulative reward in a given environment. Recent progress has witnessed success in various tasks such as Atari games \cite{mnih2015human}, Go \cite{silver2016mastering, silver2017mastering}, and robot control \cite{lillicrap2015continuous}, just to name a few, with the development of deep learning techniques. Such advances largely consist of smart, deep neural networks, which can represent action-value functions and policy functions in a reinforcement learning problem as a high-capacity function approximator. 

However, complex tasks such as robot swarm control and autonomous driving, often modeled as cooperative multi-agent learning problems, still remain unconquered due to their high scales and operational constraints such as distributed operation. The use of deep learning techniques carries through to this cooperative multi-agent reinforcement learning regime. MADDPG \cite{Lowe:MADDPG} learns distributed policy in continuous action spaces, and COMA \cite{DBLP:conf/aaai/FoersterFANW18} uses a counterfactual baseline to address the credit assignment problem.
Other related work includes CommNet \cite{sukhbaatar2016learning}, DIAL \cite{foerster2016learning}, ATOC \cite{NIPS2018_7956}, and SCHEDNET \cite{kim2018learning},
which exploit inter-agent communication in execution.

Value function factorization \cite{koller1999computing, guestrin2002multiagent} methods have been proposed to efficiently handle a joint action-value function whose complexity grows exponentially with the number of agents. This approach adopts the philosophy of centralized training with decentralized execution (CTDE) \cite{oliehoek2008optimal}, naturally motivating the method of value function factorization by learning and constructing the individual value functions of agents, such that its optimization leads to the optimization of the joint value function. At execution time, optimal action/s could be selected simply by looking up the individual value functions, without joint action-value function.

Two representative examples of this approach include VDN \cite{DBLP:conf/atal/SunehagLGCZJLSL18} and QMIX \cite{pmlr-v80-rashid18a}. In VDN, a joint action-value function is factorized via a summation of individual value functions. QMIX extends this additive value factorization to represent the joint action-value function as a monotonic function --- rather than just as a summation --- of individual value functions, covering a richer class of multi-agent reinforcement learning problems than does VDN. 
 However, these value factorization techniques still suffer structural constraints, namely, additive decomposability in VDN and monotonicity in QMIX, thereby often failing to factorize a facotrizable task. A task is factorizable if the optimal actions of the joint action-value function are the same as the optimal ones of the individual action-value functions, where additive decomposability and monotonicity are only sufficient for factorizability.  
 
 %  VDN assumes an additively decomposable joint action-value function, whereas QMIX, while slightly relaxing the assumption, still requires that each individual Q function be subject to monotonicity conditions.

\myparagraph{Contribution}
In this paper, we aim at successfully factorizing any factorizable task, and propose  
$\algoname$, which takes a different angle for factorization from VDN and QMIX.
% To this end, we first define a condition called IGM (Invidiual-Global-MAX) which states our goal of factorization of $\Qtot$ into $[Q_i]_i.$
Rather than enforcing structural constraints such as additivity and monotonicity for direct factorization, we pursue an alternative
path: transforming 
the original joint action-value function into a new one that is easily factorizable with the optimal actions in the original and the transformed joint action-value functions unchanged. \note{WJ: what is meant by "unchanged"?}
We prove that any factorizable value function is ensured to be factorized by this transform-based method. 

% \note{One more paragraph about our contribution: KH, what is the best content? We will see later.}
We instantiate the above idea with the following method of deep Q-networks. First, we propose novel neural network architectures, called $\algonamebasic$ and $\algonameadv$ that can represent much richer class of joint action-value functions than VDN and QMIX. To train this architectures, we introduce new loss functions based on the theoretical analysis for two objectives: (i) training joint action-value function, and (ii) transforming joint action-value easily factorizable. Through this, our new deep-RL framework learns individual action-value functions for factorizable tasks while adopting CTDE.
% \vspace{5cm}
% \begin{comment}
% In $\algoname,$  instead of directly factorizing the original joint action-value function $\Qtot,$ we transform it into a new joint state-action value function $\Qtot'$. We mathematically prove that, by suitably transforming: (i) $\Qtot$ and $\Qtot'$ share the optimal actions, (ii) $\Qtot'$ can be easily factorized into alternate individual value functions $[Q'_i],$ and (iii) 
% each agent $i$'s  alternate value function $Q'_i$ shares its optimal action with $Q_i,$ where $[Q_i]_i$ turns out to be factorizers of the original $\Qtot$ (see {\bf Theorem~\ref{thm:ifonlyif}}).
% An analogous interpretation from a game-theoretic perspective is that
% we alter the original game $G$ into $G'$ by modifying the original payoff functions in $G'$, so that their locally optimal strategies lead to the global optimum in $G'$, whose joint optimal strategy vector equals to that of the original game $G$. 
% Thus, in $\algoname,$ any factorizable $\Qtot$ can be factorized by adaptively determining the $\Qtot'$. $\algoname$ 
% covers an even richer class of value functions than does VDN or QMIX, thereby being amenable to a wider class of multi-agent reinforcement learning tasks.
% \end{comment}

% whose optimal actions equal those of $\Qtot,$ and allows to learn how to factorize $\Qtot'$, so that 
% individually optimizing the factorized $Q'_i$ by agents easily leads to the optimal actions for $\Qtot'.$ This is supported by our theoretical analysis (see {\bf Theorem~\ref{thm:ifonlyif}}) that  
% a well-constructed $\Qtot'$ provides the 
% {\em necessary and sufficient} condition of the individual value functions $[Q_i],$ whereas 
% the assumptions enforced by VDN and QMIX ({\em i.e.}, additivity and monotonicity) corresponds to only the {\em sufficient} condition of IGM. 
% The game-theoretic interpretation of our approach corresponds to slightly altering the original game $G$ into $G'$ by modifying individual player's payoff function in $G'$, so that their locally optimal strategies easily lead to the global optimum in $G'$, yet with the optimal joint strategy unchanged at that of $G$. 
% We construct $\Qtot'$ to be a suitable combination of the original $\Qtot$ and some regularizer, which should be learned given a game (or a multi-agent task in our context) and is responsible for replacing $G$ with $G'$ so as to removing ``bad equilibrium" ({\em i.e.}, the point different from that by IGM).   

% \begin{comment}

% Here, we propose PQMIX, capable of representing a much wider class of centralized Q functions.
% Unlike VDN or QMIX, PQMIX factorizes the centralized Q function into an additive sum with penalized regularization. We mathematically prove that this form of factorization covers more generalized scenarios of cooperative multi-agent tasks than those handled by previous works. We then present a simple game that can be well-treated by PQMIX, but not by VDN or QMIX. 

% We alter the payoff structure of some well-known games to reflect more realistic characteristics that necessitate cooperative behavior. These alterations are designed such that exhibiting a non-cooperative behavior would drive the agents to fall in a suboptimal local Nash equilibrium. We demonstrate with simulations that with a greater extent of the said alteration, PQMIX outperforms previous works by a larger margin. We take this empirical evidence to argue that multi-agent reinforcement learning problems requiring cooperative behavior are better addressed by PQMIX than by VDN or QMIX. \note{more sentences. WJ: more sentences added 0921}. 
% % a structure that can operate in more general environments. For all cases where optimal action set of individual action-value functions is same as optimal action of centralized action-value function, PQMIX ensures that learning is possible. 
% \end{comment}

We demonstrate the performance of our algorithm by comparing it against VDN and QMIX in three environments. First, we confirm through a theoretical analysis that $\algoname$ outperforms its predecessors in a simple matrix game. It is shown that for a class of matrix games satisfying a set of conditions, VDN and QMIX do not select optimal action/s in certain matrix games, but that $\algoname$ learns optimal action/s in every matrix game. We then observe a similarly desirable cooperation-inducing tendency of $\algoname$ in more complex environments: modified predator-prey games and Multi-domain Gaussian Squeeze tasks. In particular, we show that the performance gap between $\algoname$ and VDN/QMIX increases with environments having more pronounced non-monotonic characteristics.  


==> 5.method_backup.tex <==
\section{$\algoname$: Learning to Factorize with Regularization \note{2 page}}

Now we propose a new approach called $\algoname$, which have advantages of CTDE like VDN and QMIX, but can represent a much richer class of action-value functions with regularization. We additionally make a centralized regularization function $F(\bm{\tau},\bm{u})$, which transform original centralized $\Qtot$ to factorable $\Qtot'$:
\begin{align}
\Qtot(\bm{\tau},\bm{u}) + F(\bm{\tau},\bm{u}) &= \Qtot'(\bm{\tau},\bm{u}) = \sum_{i=1}^n Q'_i(\tau_i, u_i), \\
\arg\max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}) &= \arg\max_{\bm{u}} \Qtot'(\bm{\tau},\bm{u}), \label{eq:argmax_cond}
\end{align}
where $Q'_i(\tau_i, u_i)$ is factorized individual action-value functions from $\Qtot'$. With \ref{eq:argmax_cond}, $\algoname$ allows optimal action selection by greedy decentralized action selection. Key to our method is when the transforming is possible and how to find appropriate regularizer $F(\bm{\tau},\bm{u})$.

\subsection{{\bf IGM} Condition}

We first define the condition, called {\bf IGM} (Individual-Global-Max), which, if met, implies that the global action-value function is well-factorized.  
\begin{defi}
For a global action-value function $\Qtot: \set{T}^n \times \set{U}^n \mapsto \real$, where $\bm{\tau} \in \set{T}^n$ is a joint action-observation histories, we say that a collection of the individual functions $[Q_i: \set{T}_i \times \set{U}_i \mapsto \real]_{i=1}^N,$ satisfies {\bf IGM}, if the following holds:
\begin{align}
\label{eq:max_cond}
\arg\max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}) & = 
\begin{pmatrix}
\arg\max_{u_1} Q_1(\tau_1, u_1) \\
\vdots \\
\arg\max_{u_n} Q_n(\tau_n, u_n)
\end{pmatrix}.
\end{align}
\end{defi}

% We aim at ensuring the condition, which we call IMC (Individual Max Condition) that a global argmax performed on $\Qtot$ yields
% the same result as a set of individual argmax operations
% performed on each $Q_a$:
We now derive the necessary and sufficient condition of $[Q_i]$ for satisfying {\bf IGM}, 
which provides a useful guideline on how to factorize the global joint action-value function $\Qtot.$ To this end, we first denote the global and individual value functions as $\Vtot(\bm{\tau}) = \max_{\bm{u}} \Qtot(\bm{\tau},\bm{u})$ and $V_i({\tau_i}) = \max_{{u_i}} Q_i({\tau_i},{u_i}).$ Then, we define a regularizer function $F(\bm{\tau},\bm{u})$ as follows:

\begin{align}
\label{eq:define_F}
F(\bm{\tau},\bm{u}) &:= \sum_{i=1}^n (Q_i(\tau_i, u_i) - V_i({\tau_i}))   \notag\\
& - ( \Qtot(\bm{\tau},\bm{u}) - \Vtot(\bm{\tau})). 
\end{align}

Then, we introduce two functions $Q'_i$ and $\Qtot'$, modified ones from $Q_i$ and $\Qtot$, defined as:
\begin{align}
    Q'_i(\tau_i, u_i) & := Q_i(\tau_i, u_i) - V_i({\tau_i}), \label{eq:q_prime} \\ 
\Qtot^{\prime}(\bm{\tau},\bm{u}) & := \Qtot(\bm{\tau},\bm{u}) - \Vtot(\bm{\tau})  + F(\bm{\tau},\bm{u}), \label{eq:define_qtprime}
\end{align}
where from \eqref{eq:define_F} and \eqref{eq:define_qtprime} we can rewrite $\Qtot'$ as:
\begin{align}
\label{eq:qtotagain}
\Qtot'(\bm{\tau},\bm{u}) = \sum_{i=1}^n Q'_i(\tau_i, u_i). 
\end{align}

% \begin{comment}
% Next, we define the following two variant functions of $Q_i$ and $\Qtot$ as follows: 
% \begin{align}
%     Q'_i(\tau_i, u_i) & := Q_i(\tau_i, u_i) - V_i({\tau_i}), \label{eq:q_prime} \\ 
% \Qtot'(\bm{\tau},\bm{u})& := \sum_{i=1}^n Q'_i(\tau_i, u_i) 
% \end{align}
% % \begin{align}
% % u^i_{\max} &= \arg\max_{u^{i}}Q_i(\tau^i,u^{i}), \hspace{0.5cm}
% % \Vtot(\bm{\tau}) = \max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}), \hspace{0.5cm} 
% % V_i({\tau^{i}}) = \max_{{u^{i}}} Q_i({\tau^{i}},{u^{i}})
% % \end{align}(3
% % Now, for a given $\alpha >0,$ we define the following two functions:
% Then, by denoting $F(\bm{\tau},\bm{u})$ as
% \begin{align}
% \label{eq:define_F}
% F(\bm{\tau},\bm{u}) &:= \sum_{i=1}^n Q'_i(\tau_i, u_i) - ( \Qtot(\bm{\tau},\bm{u}) - \Vtot(\bm{\tau})), 
% \end{align}
% we can rewrite $\Qtot'$ as:
% \begin{align}
% \label{eq:define_qtprime}
% \Qtot^{\prime}(\bm{\tau},\bm{u}) = \Qtot(\bm{\tau},\bm{u}) - \Vtot(\bm{\tau})  + F(\bm{\tau},\bm{u}).
% \end{align}
% % and thus 
% % $\arg\max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}) = \arg\max_{\bm{u}} \Qtot'(\bm{\tau},\bm{u}).$ 
% \end{comment}

% Denote $\bm{u}^{\max} = [u^{\max}_i]_{i=1}^N,$ where 
% $u^{\max}_i = \arg\max_{u^{i}}Q_i(\tau_i,u_i).$ Theorem~\ref{thm:ifonlyif} states the necessary and sufficient condition of a collection of individual value functions $[Q_i]_{i=1}^N$ for the {\bf IGM} condition. 

We now present sufficient and necessary condition of regularizer function $F(\bm{\tau},\bm{u})$ to satisfy {\bf IGM} condition.

\begin{theorem}
\label{thm:ifonlyif}
For a given global action-value function $\Qtot$ and a collection of individual 
action-value functions $[Q_i]_{i=1}^N,$ the following condition on $F$ is if and only if {\bf IGM} condition holds: 
\begin{align}
\label{eq:regular_cond}
F(\bm{\tau},\bm{u}) &= 
\begin{cases}
    0,& \text{\rm if} \quad \bm{u} = \bm{u}^{\max}\\
    \geq 0,              & \text{\rm otherwise},
\end{cases}
\end{align}
where ${u}^{\max}_{i} = \arg\max_{u_{i}}Q_i(\tau_i,u_i)$, and greedy action $\bm{u}^{\max} = [{u}^{\max}_{i}]_{i=1}^N.$
\end{theorem}

A full discussion and a proof is given in Appendix.
% To prove sufficiency, $F(\bm{\tau},\bm{u}^{\max})$ is the minimum value and $\Qtot'(\bm{\tau},\bm{u}^{\max})$ is the maximized value for given $\tau$. So it is easily proved by $\bm{u}^{\max} = \arg\max_{\bm{u}} \Qtot(\bm{\tau},\bm{u})$. Additionally, for necessity, we can find linearly scaled $Q_i$ to be small enough, still satisfying the {\bf IGM} condition. There always exist scaled $Q_i$ to make $F(\bm{\tau},\bm{u})$ is greater than or equal to zero.
% \begin{proof}

% From the definitions, the followings hold: (i) $Q'_i(\tau_i, u^{\max}_i) = 0$ and (ii) $\Qtot(\bm{\tau},\bm{u}) = \Vtot(\bm{\tau}) - F(\bm{\tau},\bm{u}) +  \sum_{i=1}^n Q'_i(\tau^i, u^i)$. Further $\Qtot(\bm{\tau},\bm{u}_{\max}) = \Vtot(\bm{\tau}) - F(\bm{\tau},\bm{u}_{\max}) +  \sum_{i=1}^n Q'_i(\tau^i, u_{\max}^i) = \Vtot(\bm{\tau})$ and $\Qtot(\bm{\tau},\bm{u}) = \Vtot(\bm{\tau}) - F(\bm{\tau},\bm{u}) +  \sum_{i=1}^n Q'_i(\tau^i, u^i) \leq  \Vtot(\bm{\tau})$. Therefore we can show the {\bf IGM} holds.

% To prove necessity, we will now show it must be the case that $F(\bm{\tau},\bm{u})$ satisfies condition \eqref{eq:regular_cond}. We can rewrite $F(\bm{\tau},\bm{u})$ as $F(\bm{\tau},\bm{u}) = (\Vtot(\bm{\tau}) - \Qtot(\bm{\tau},\bm{u})) - \sum_{i=1}^n (V_i({\tau^{i}}) - Q_i(\tau^i, u^i))$. 
% Then by definition and condition {\bf IGM}, $F(\bm{\tau},\bm{u}_{\max}) = 0$. Further, we can find linearly scaled $Q_i$ to be small enough, still satisfying the {\bf IGM} condition so that $F(\bm{\tau},\bm{u})$ is greater than or equal to zero.

% \end{proof}
We now present how we use {\bf Theorem~\ref{thm:ifonlyif}} to facilitate the factorization into the each agent's individual local action-value function, which naturally leads to the optimization of the global joint action-value function. Our goal is to find $[Q_i]$ that satisfies {\bf IGM} for a given $\Qtot$. 
It becomes challenging to find such 
$[Q_i]$ unless the underlying game has special properties such as additivity (as in VDN) or monotonicity 
(as in QMIX). Our novel idea is to find $[Q_i]$ satisfying {\bf IGM} indirectly by constructing them so as to meet an alternate condition expressed by $F$ (as in \eqref{eq:define_F} and \eqref{eq:regular_cond}), which turns out to be both necessary and sufficient for {\bf IGM} by {\bf Theorem~\ref{thm:ifonlyif}}. 
Necessity in {\bf Theorem~\ref{thm:ifonlyif}} states that for given $\Qtot$,
$Q_i$ satisfies {\bf IGM}, if it satisfies \eqref{eq:regular_cond}. 
Then, if we construct $[Q_i]$ to meet \eqref{eq:regular_cond}, then those $[Q_i]$ automatically become the individual action-value functions that factorize $\Qtot$.
Sufficiency in {\bf Theorem~\ref{thm:ifonlyif}} guarantees that that there always exists 
$F$ as defined in \eqref{eq:define_F} satisfying \eqref{eq:regular_cond}. 


% It is easy to find such $Q_i$ if the game has special properties such as additivity of monotonicity. However, it is impossible to find $Q_i$ in general for games that satisfy {\bf IGM} through existing methods. Our novel idea is not to find the $Q_i$ that satisfies {\bf IGM} directly, but to find the $Q_i$ to satisfy the new condition that is equivalent to satisfy the {\bf IGM}.

% Given $\Qtot$ and $Q_i$, the new condition is represented by \eqref{eq:define_F} and \eqref{eq:regular_cond}. The new condition has the same meaning as the existing condition {\bf IGM}, and is easy to handle practically. Theorem~\ref{thm:ifonlyif} tells how the two conditions are connected. The necessary condition of our Theorem~\ref{thm:ifonlyif} is that $\Qtot$ and $Q_i$ satisfy {\bf IGM}, if $\Qtot$ and $Q_i$ satisfy \eqref{eq:regular_cond}. Then, if we make $Q_i$ satisfies \eqref{eq:regular_cond}, then such $Q_i$ automatically becomes a function that factorizes $\Qtot$. Also, sufficient condition proves that there is always $F$ satisfies condition \eqref{eq:define_F}. We will introduce more details about how to use this condition in Section~\ref{sec:method}.

The meaning of $F$ can be understood through the modified action-value functions $\Qtot'$ and $Q_i'$. Given $\Qtot$ and $Q_i$, $\Qtot'$ corresponds to a kind of {\em regularized} global action-value function by taking the summation of $\Qtot$ and $F$ as in \eqref{eq:define_qtprime}.
By adding $F$ to $\Qtot$, $\Qtot$ is transformed to $\Qtot'$ that is additively decomposed to $[Q_i']$. We note that new action-value functions $\Qtot'$ and $[Q_i']$ have the same optimal solutions as $\Qtot$ and $[Q_i]$, respectively, by \eqref{eq:q_prime},  \eqref{eq:define_qtprime}, and the condition of $F$ in \eqref{eq:regular_cond}. 
This enables us to easily learn how to factorize $\Qtot$ by changing our angle through a well-constructed regularizer $F.$

% modifying the shape of the existing function $\Qtot$, but the optimal action is maintained.
% In addition, we can confirm that the newly created $\Qtot'$ and $Q_i'$ through  have the same optimal as existing $\Qtot$ and $Q_i$ by condition \eqref{eq:regular_cond}. Therefore, $F$ acts as a regularizer, so it is easy to learn 


% For games that satisfy {\bf IGM} conditions, $\Qtot$ is generally not possible to completely factorize with VDN and QMIX. Instead of factorizing this $\Qtot$, we defined a new joint Q-function $\Qtot'$ which is easy to factorize. $\Qtot$ has the same optimal action as $\Qtot$, and it can be represented in the summation of new individual Q-functions $Q_i'$. Also, $Q_i'$ has the same optimal action as $Q_i$. The necessary condition of Theorem~\ref{thm:ifonlyif} shows that there exists a new $\Qtot'$ and $Q_i'$ for all games that satisfy {\bf IGM} condition. The sufficient condition tell us how to find $\Qtot'$, and the condition is given through the form of regularizer $F(\bm{\tau},\bm{u})$.

\begin{figure*}[ht]
\begin{subfigure}[t]{.58\textwidth}
  \includegraphics[width=\linewidth]{figure/qreg_q1}
  \caption{Individual Action-Value Networks Structure}
  \label{fig:rnet1}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}[t]{.40\textwidth}
  \includegraphics[width=\linewidth]{figure/rnn.pdf}
  \caption{Agent Network Structure}
  \label{fig:rnn}
\end{subfigure}\hspace*{\fill}
\caption{$\algoname$ Architecture}
\label{fig:NN}
\end{figure*}


\begin{figure*}[h]
  \centering
 \includegraphics[width=0.92\textwidth]{figure/qreg_q2}
\caption{$\algoname$ Architecture: Global action-value networks}
  \label{fig:NN2}
\end{figure*}

\begin{figure*}[ht]
\begin{subfigure}[t]{.45\textwidth}
  \includegraphics[width=\linewidth]{figure/vdn.pdf}
  \caption{VDN Structure}
  \label{fig:vdn}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}[t]{.53\textwidth}
  \includegraphics[width=\linewidth]{figure/qmix}
  \caption{QMIX Structure}
  \label{fig:qmix}
\end{subfigure}\hspace*{\fill}
\caption{VDN and QMIX Architecture}
\label{fig:NN3}
\end{figure*}

% \begin{figure*}[h]
%   \centering
%  \includegraphics[width=0.92\textwidth]{figure/QREG}
% \caption{$\algoname$ Architecture}
%   \label{fig:NN}
% \end{figure*}

\subsection{Method}\label{sec:method}

% \begin{figure}
%   \includegraphics[width=1\linewidth]{figure/pqmix_temp.pdf}
%   \caption{Provisional pqmix architecture}
%   \label{fig:pqmix}
% \end{figure}
% \begin{comment}
  

% \begin{figure*}[ht]
% \begin{subfigure}[t]{.32\textwidth}
%   \includegraphics[width=\linewidth]{figure/rnn.pdf}
%   \caption{Individual Action-Value Network}
%   \label{fig:rnn}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}[t]{.27\textwidth}
%   \includegraphics[width=\linewidth]{figure/rnet1.pdf}
%   \caption{Soft Regularization Network}
%   \label{fig:rnet1}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}[t]{.40\textwidth}
%   \includegraphics[width=\linewidth]{figure/rnet2.pdf}
%   \caption{Hard Regularization Network}
%   \label{fig:rnet2}
% \end{subfigure}\hspace*{\fill}
% \caption{$\algoname$ architecture}
% \label{fig:NN2}
% \end{figure*}
% \end{comment}



In this section, we propose a new method of value function factorization, which we call $\algoname$, inspired by our theoretical analysis in {\bf Theorem~\ref{thm:ifonlyif}}.  In centralized Q-learning, we learn $\Qtot$ through function approximators such as neural networks with a centralized trainer. In this paper, we propose $\algoname$ to approximate and factorize $\Qtot$, consisting of three separate estimators: (i) a action-value function for $\Qtot'$, which can be factorized into individual action-value networks $Q_i$, (ii) a value network for $\Vtot$, and (iii) a regularization network for $F$. Figure~\ref{fig:NN} shows the overall structure of $\algoname$ and of three estimators inside $\algoname$.
Since we construct each module to satisfy the condition \eqref{eq:regular_cond} from {\bf Theorem~\ref{thm:ifonlyif}}, $\Qtot'$ can be factorized into individual action-value function $Q_i$ and also satisfy $\arg\max\Qtot' = \arg\max\Qtot.$
This ensures that we train decentralized policies at individual agents in a centralized fashion, which follows the CTDE paradigm.
% We fist present the architecture of $\algoname$ first, followed by that of three estimators. 

We generate three modules of $\algoname$ as follows.
\begin{align*}
&\text{\bf Action-value networks} \  f_{\text{q}}: (\tau_i,u_i) \mapsto Q'_i, \cr \quad
&\text{\bf Regularization network} \  f_{\text{r}}: (\vec{\tau}, \vec{u}) \mapsto F, \cr
  &\text{\hspace{0cm}} \text{\bf Value network} \  f_{\text{v}}: \vec{\tau} \mapsto
    \Vtot. 
\end{align*}

As $\Qtot$ is learned, the estimators are updated through the following equation $\Qtot = \Vtot + \Qtot' - F(\bm{\tau},\bm{u})$. If $Q_i, \Vtot$, and $F$ are trained well so as to satisfy the condition in \eqref{eq:regular_cond}, then the learned individual action-value functions are trained to also satisfy {\bf IGM}, thus factorizing $\Qtot$ well. This ensures that we train decentralized policies at individual agents in a centralized fashion. Figure~\ref{fig:NN} shows the overall structure of $\algoname$ and those of three modules inside $\algoname$. $\Qtot$ is learned through a combination of three modules. And we will introduce each network one by one.

\paragraph{Individual action-value networks} For each agent, there is an action-value network that takes its own action-observation history $\tau^i$ as input and outputs action-values $Q_i$. This action-value network is used for two purposes. From the agents' perspective, each agent can determine its own action by calculating action-value for a given $\tau^i$. From perspective of a centralized trainer, it is also used to calculate $\Qtot'$, one of modules that form $\Qtot$.

% \begin{figure}[h!]
%   \centering
%  \includegraphics[width=0.9\columnwidth]{figure/qnet}
% \caption{Action-Value Network}
%   \label{fig:qnet}
% \end{figure}

\paragraph{Value network} Finally, value network is responsible for computing scalar state-value, like $V(s)$ in the dueling network \citep{wang2016dueling}. The state-value is independent of selected action for a given $\bm{\tau}$. Thus, value network does not contribute to determine action, and is just used to calculate $\Qtot$.

\subsection{Training Regularization Network}\label{sec:regular}

We now present the regularization network, which is key to our method. In order to successfully factorize $\Qtot$ into individual action-value functions $Q_i$ ({\em i.e.}, $Q_i$ satisfies {\bf IGM}), $F$ should satisfy condition \eqref{eq:regular_cond}. We propose two structures: (i) soft regularization network and (ii) hard regularization network that approximates $F$. 

\paragraph{Soft regularization network} The soft regularization network has a module, which computes $F(\bm{\tau},\bm{u})$. $F(\bm{\tau},\bm{u})$ is always greater than or equal to 0 by absolute operation. To make regularization network satisfies condition \eqref{eq:regular_cond}, we propose objective can be written as:
\begin{align*} 
&L_F(\vec{\tau}, \vec{u}^{\max}; \bm{\theta}):= F(\vec{\tau},\vec{u}^{\max};\theta)^{2}.
\end{align*}

The input $\vec{u}^{\max}$ to calculate the loss is from individual action-value functions.  If the loss is zero, we can verify that $F$ equals to 0 when $\bm{u}=\bm{u}^{\max}$. In this way, we can guarantee that condition \eqref{eq:regular_cond} holds.

% \begin{figure}[h!]
%   \centering
%  \includegraphics[width=0.7\columnwidth]{figure/rnet}
% \caption{Regularization Network}
%   \label{fig:rnet}
% \end{figure}

% We construct the regularization network to output $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{u}^{\max}))^2$.
% For any function $R$, we can verify that $F(\bm{\tau},\bm{u})$ is always greater than or equal to 0 and that $F$ equals to 0 when $\bm{u}=\bm{u}^{\max}$. In this way, during training $F$, $\Qtot'$, and $\Vtot$, we can always guarantee that condition \eqref{eq:regular_cond} holds.



% \begin{figure}[h!]
%   \centering
%  \includegraphics[width=0.5\columnwidth]{figure/vnet}
% \caption{Value Network}
%   \label{fig:vnet}
% \end{figure}

During centralized training, we use the algorithm introduced in DQN \citep{mnih2015human} to update networks.
We maintain the target network and replay buffer, which store the sample $(\vec{\tau},\vec{u},r, \vec{\tau}')$, and we update the parameters to minimize the loss function defined as:
\begin{align*} 
L(\vec{\tau}, \vec{u}, r, \vec{\tau}'; \bm{\theta}):&=
L_Q + \lambda L_F
, \cr \quad
L_Q(\vec{\tau}, \vec{u}, r, \vec{\tau}'; \bm{\theta}):&= (\Qtot(\vec{\tau},\vec{u};\theta) - y(\vec{\tau}, \vec{u}, r, \vec{\tau}'; \bm{\theta}))^{2},\cr \quad
L_F(\vec{\tau}, \vec{u}^{\max}; \bm{\theta}):&= F(\vec{\tau},\vec{u}^{\max};\theta)^{2},
\label{eq:lossF} 
\end{align*} 
where $y(\vec{\tau}, \vec{u}, r, \vec{\tau}'; \bm{\theta}) = (r + \gamma \max_{\vec{u}'} \Qtot(\vec{\tau}', \vec{u}';\theta '))$ and $\lambda$ is hyperparameter. At the end of learning, each agent is controlled in a decentralized fashion using only its own individual action-value function.

\paragraph{Hard regularization network} Now we present additional method to implement regularization network. The network computes $R(\bm{\tau},\bm{u})$ instead of $F(\bm{\tau},\bm{u})$ by taking $\bm{\tau}, \bm{u}$ as input. For any function $R$, we can confirm $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{u}_{\max}))^2$ is always greater than or equal to 0 , and it is 0 when $\bm{u}=\bm{u}_{\max}$. This is consistent with condition \eqref{eq:regular_cond} of $F$, so we can learn $F(\bm{\tau},\bm{u})$ as we update $R(\bm{\tau},\bm{u}$). 


\paragraph{Comparison}

A key feature of the soft regularization network is its smoothness. Soft regularization network is not always satisfied the condition \eqref{eq:regular_cond}, but the network has more representational complexity than hard regularization network and it is differentiable.
On the contrary, hard regularization network is always satisfied the condition \eqref{eq:regular_cond}, but representational complexity is restricted during training. Also, there is a problem that argmax operation is non differentiable.

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[!ht]
    \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$u_1$}{$u_2$}& A & B & C\\ \hline \hline
        A & \textbf{8}& -12 & -12 \\ \hline
        B & -12 & 0 & 0 \\ \hline
        C & -12 & 0 & 0 \\ \hline
        \end{tabular}
        \subcaption{Non-monotonic cooperative matrix game}
        \label{table:p7orig}
    \end{minipage}%
        \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
            \hline
            \backslashbox{$Q_1$}{$Q_2$} & -3.14(A) & \textbf{-2.29}(B) & -2.41(C)\\ \hline \hline
            -2.29(A) & -5.42  & -4.57 & -4.70 \\ \hline
            -1.22(B) & -4.35 & -3.51 & -3.63 \\ \hline
            \textbf{-0.73}(C) & -3.87 & \textbf{-3.02} & -3.14 \\ \hline
        \end{tabular}
        \subcaption{$Q_1, Q_2,$ and $\Qtot$ for VDN}
        \label{table:matrix-vdn}
    \end{minipage}
    \begin{minipage}{.48\linewidth}
      \centering
         \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$Q_1$}{$Q_2$} & -0.92(A) & 0.00(B) & \textbf{0.01}(C)\\ \hline \hline
        -1.02(A) & -8.08  & -8.08 & -8.08 \\ \hline
        \textbf{0.11}(B) & -8.08 & 0.01 & \textbf{0.03} \\ \hline
        0.10(C) & -8.08 & 0.01 & 0.02 \\ \hline
        \end{tabular}
        \subcaption{$Q_1, Q_2,$ and $\Qtot$ for QMIX}
        \label{table:matrix-qmix}
    \end{minipage}%
        \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$Q_1$}{$Q_2$} & \textbf{4.16}(A) & 2.29(B) & 2.29(C)\\ \hline \hline
        \textbf{3.84}(A) & \textbf{8.00}  & 6.13 & 6.12 \\ \hline
        -2.06(B) & 2.10 & 0.23 & 0.23 \\ \hline
        -2.25(C) & 1.92 & 0.04 & 0.04 \\ \hline
        \end{tabular}
        \subcaption{$Q_1, Q_2,$ and $\Qtot'$ for $\algoname$}
        \label{table:matrix-qreg}
    \end{minipage}
    \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$u_1$}{$u_2$}& A & B & C\\ \hline \hline
        A & \textbf{8.00}  & -12.02 & -12.02 \\ \hline
        B & -12.00 & 0.00 & 0.00 \\ \hline
        C & -12.00 & 0.00 & -0.01 \\ \hline
        \end{tabular}
        \subcaption{$\Qtot$ for $\algoname$}
        \label{table:matrix-qreg'}
    \end{minipage}%
    \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$u_1$}{$u_2$}& A & B & C\\ \hline \hline
        A & \textbf{0.00}  & 18.14 & 18.14 \\ \hline
        B & 14.11 & 0.23 & 0.23 \\ \hline
        C & 13.93 & 0.05 & 0.05 \\ \hline
        \end{tabular}
        \subcaption{$F$ for $\algoname$}
        \label{table:matrix-F}
    \end{minipage}
        \caption{Payoff matrix of the one-step game and reconstructed $\Qtot$ results on the game }
\end{table*}

\subsection{Matrix game}

To compare the performance of the representational complexity of VDN , QMIX and $\algoname$, we devise a matrix game with two agents. The matrix game is the simplest form of cooperative multi-agent problem. The game is a one-step game with only one state and three actions per agent as shown in Table~\ref{table:p7orig}. The team reward is determined is through a payoff matrix and joint action. We trained VDN, QMIX, and QREG through a full exploration for 20,000 episodes in two matrix games. Detailed settings are introduced in Appendix





% \begin{table}[!ht]
% \caption{Non-monotonic cooperative matrix game}
% \label{table:p7orig}
% \vskip 0.15in
% \begin{center}
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         & A & B & C\\ \hline \hline
%         A & \textbf{8}& -12 & -12 \\ \hline
%         B & -12 & 0 & 0 \\ \hline
%         C & -12 & 0 & 0 \\ \hline
%     \end{tabular}
% \end{center}
% \vskip -0.1in
% \end{table}


% \begin{table*}[!ht]
% \caption{Non-monotonic cooperative matrix game}
% \label{table:p7orig2}
% \vskip 0.15in
% \begin{center}
%     \begin{tabular}{|P{1.3cm}||P{1.5cm}|P{1.5cm}|P{1.5cm}|}
%         \hline
%         \backslashbox{$Q_1$}{$Q_2$} & A:-3.14 & B:\textbf{-2.29} & C:-2.41\\ \hline \hline
%         -2.29 & -5.42  & -4.57 & -4.70 \\ \hline
%         -1.22 & -4.35 & -3.51 & -3.63 \\ \hline
%         \textbf{-0.73} & -3.87 & \textbf{-3.02} & -3.14 \\ \hline
%     \end{tabular}
% \subcaption{$Q_1, Q_2,$ and $\Qtot$ for VDN}
% \label{table:matrix-vdn}
%     \begin{tabular}{|P{1.3cm}||P{1.5cm}|P{1.5cm}|P{1.5cm}|}
%         \hline
%         \backslashbox{$Q_1$}{$Q_2$} & -0.92 & 0.00 & \textbf{0.01}\\ \hline \hline
%         -1.02 & -8.08  & -8.08 & -8.08 \\ \hline
%         \textbf{0.11} & -8.08 & 0.01 & \textbf{0.03} \\ \hline
%         0.10 & -8.08 & 0.01 & 0.02 \\ \hline
%     \end{tabular}
% \subcaption{$Q_1, Q_2,$ and $\Qtot$ for QMIX}
% \label{table:matrix-qmix}
% \medskip
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         \backslashbox{$Q_1$}{$Q_2$} & \textbf{4.16} & 2.29 & 2.29\\ \hline \hline
%         \textbf{3.84} & \textbf{8.00}  & 6.13 & 6.12 \\ \hline
%         -2.06 & 2.10 & 0.23 & 0.23 \\ \hline
%         -2.25 & 1.92 & 0.04 & 0.04 \\ \hline
%     \end{tabular}
% \subcaption{$Q_1, Q_2,$ and $\Qtot'$ for $\algoname$}
% \label{table:matrix-qreg}
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         & A & B & C\\ \hline \hline
%         A & \textbf{0.00}  & 18.14 & 18.14 \\ \hline
%         B & 14.11 & 0.23 & 0.23 \\ \hline
%         C & 13.93 & 0.05 & 0.05 \\ \hline
%     \end{tabular}
% \subcaption{$F$ for $\algoname$}
% \label{table:matrix-F}
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         & A & B & C\\ \hline \hline
%         A & \textbf{8.00}  & -12.02 & -12.02 \\ \hline
%         B & -12.00 & 0.00 & 0.00 \\ \hline
%         C & -12.00 & 0.00 & -0.01 \\ \hline
%     \end{tabular}
% \subcaption{$\Qtot$ for $\algoname$}
% \label{table:matrix-qreg'}
% \end{center}
% \vskip -0.1in
% \end{table*}



Table~\ref{table:matrix-vdn} and Table~\ref{table:matrix-qmix} illustrate that vdn and qmix learned the sub-optimal policy. However, our algorithm restored $\Qtot$ accurately and learned $\Qtot'$, which is easy to factorize as shown in Table~\ref{table:matrix-qreg} and Table~\ref{table:matrix-qreg'}.


% \textbf{additional design }

% \textbf{Computational Complexity}
% Computational complexity of QMIX and $\algoname$ can be qualitatively compared. Typically, representational complexity and computational complexity are in a trade-off relationship. Comparing QMIX with VDN, representational and computational complexity increase together because summation part of VDN is replaced by monotonic neural network. However, even if $\algoname$ has larger representational complexity than QMIX, computational complexity is not always larger. QMIX constructs that weight of a monotonic neural network through extra state information and another network, hypernetworks. Without weight sharing, computational complexity of hypernetworks increases dramatically as neural networks become deeper. Otherwise, $\algoname$ can use extra state information without using hypernetworks.

% We now present the regularization network which is a key part of our method. We construct $F$ to satisfy \eqref{eq:regular_cond} and update $Q_i$ and $F$ together. The regularization network computes $R(\bm{\tau},\bm{u})$ instead of $F(\bm{\tau},\bm{u})$ by taking $\bm{\tau}, \bm{u}$ as input, as shown in Figure~\ref{fig:rnet}. For any function $R$, we can confirm $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{u^{\max}}))^2$ is always greater than or equal to 0 and is 0 when $\bm{u}=\bm{u^{\max}}$. This is consistent with condition \eqref{eq:regular_cond} of $F$, so we can learn $F(\bm{\tau},\bm{u})$ as we update $R(\bm{\tau},\bm{u}$). 

% Instead of  doing this, we can consider other method that update $Q_i$ by designing loss function to satisfy \eqref{eq:regular_cond}. The advantage of this method is that the relationship between $F$ and $Q_i$ becomes clear because $F$ is expressed through $Q_i$ without using independent networks for $F$. Also, the amount of computation can be reduced because no additional networks are used. However, we already have a loss functions to learn $\Qtot$, so it is difficult to balance two loss functions at the same time. Therefore, we designed the regularization network using the previous method. 


% \begin{comment}
%   In this section, we propose a new method of value function factorization, which we call $\algoname$, inspired by our theoretical analysis in Theorem~\ref{thm:ifonlyif}.
% In the centralized Q-learning, we learn $\Qtot$ through function approximators such as  neural networks with a centralized trainer. We learn $\Qtot'$ so as to be factorized and also to satisfy $\arg\max\Qtot' = \arg\max\Qtot.$ Our network includes three separate estimators: (i) individual action-value networks for $Q_1, Q_2, ... Q_n$, (ii) value network for $\Vtot$, and (iii) regularization network for $F$. As $\Qtot$ is learned, the estimators are updated through the following equation $\Qtot = \Vtot + \Qtot' - F(\bm{\tau},\bm{u})$. If $Q_i, \Vtot$, and $F$ are trained well so as to satisfy the condition in \eqref{eq:regular_cond}, then the learned individual action-value functions are trained to also satisfy {\bf IGM}, thus factorizing $\Qtot$ well. This ensures that we train decentralized policies at individual agents in a centralized fashion. Figure~\ref{fig:NN} shows the overall structure of $\algoname$ and those of three modules inside $\algoname$. $\Qtot$ is learned through a combination of three modules, as depicted in Figure~\ref{fig:qgnet}. And we will introduce each network one by one.


% \subsection{Centralized training with decentralized execution}
% We consider a centralized training with decentralized execution, where the learning algorithm has access to all local action-observation histories $\bm{\tau}$ in conjunction with the global state $\bm{s}$, but each agent's learned policy can condition only on its own action-observation history $\tau_i$.

% Update process proceeds end-to-end to minimize TD-error from centralized action-value function. Like the standard DQN, target network and replay buffer are used, and all networks are trained at once to minimize global loss function. At the end of learning, each agent is controlled decentralized using only its individual action-value function.

% \subsection{Regularization network} 

% First, regularization network is a key part of our method. We construct $F$ to satisfy \eqref{eq:regular_cond} and update $Q_i$ and $F$ together. The regularization network computes $R(\bm{\tau},\bm{u})$ instead of $F(\bm{\tau},\bm{u})$ by taking $\bm{\tau}, \bm{u}$ as input, as shown in Figure~\ref{fig:rnet}. For any function $R$, we can confirm $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{u}^{\max}))^2$ is always greater than or equal to 0 and is 0 when $\bm{u}=\bm{u}^{\max}$. This is consistent with condition \eqref{eq:regular_cond} of $F$, so we can learn $F(\bm{\tau},\bm{u})$ as we update $R(\bm{\tau},\bm{u}$). 

% Instead of  doing this, we can consider other method that update $Q_i$ by designing loss function to satisfy \eqref{eq:regular_cond}. The advantage of this method is that the relationship between $F$ and $Q_i$ becomes clear because $F$ is expressed through $Q_i$ without using independent networks for $F$. Also, the amount of computation can be reduced because no additional networks are used. However, we already have a loss functions to learn $\Qtot$, so it is difficult to balance two loss functions at the same time. Therefore, we designed the regularization network using the previous method. 


% \subsection{Individual action-value and value networks} Figure~\ref{fig:qnet} illustrates structure of individual action-value networks. For each agent, there is an action-value network that takes its own action-observation history $\tau^i$ as input and outputs action-values $Q_i$. This action-value network is used for two purposes. From the agents' perspective, each agent can determine its own action by calculating action-value for a given $\tau^i$. From perspective of a centralized trainer, it is also used to calculate $\Qtot'$, one of modules that form $\Qtot$.
% Finally, value network is responsible for computing scalar state-value as illustrated in Figure~\ref{fig:vnet} like $V(s)$ in the dueling network \citep{wang2016dueling}. The state-value is independent of selected action for a given $\bm{\tau}$. Thus, value network does not contribute to determine action, and is just used to calculate $\Qtot$.

% \end{comment}



% \note{overall view}
% This section introduces general framework of $\algoname$ architecture. The neural network architecture we propose is decomposed into individual action-value networks and penalty networks. Figure shows the overall settings. Individual action-value networks are used to select action for each agent. Given action-observation histories of each agents, individual action-value networks compute action-value function. 

% \note{penalty network explanation}
% Penalty networks is the key part of our method. Penalty network takes as state and set of actions, and generates penalty value. Penalty term is determined by difference between two outputs of the penalty network. One output is for the selected action and the other is for the argmax action. So, if every agent chooses its argmax action, then two outputs are same and penalty term becomes zero. In this case, Centralized action-value function is decomposed into summation of individual action-value functions. On the other hand, if some agents select different actions, then penalty term is greater than zero. Thus, we can see that when each agent selects its argmax action, the centralized action-value function is maximized.

% \note{representational complexity or expressive power}
% Expressive power of our neural network architecture can be confirmed as follows. Intuitively, if the output of the penalty network is always 0, our network is the same as VDN. Moreover, $\algoname$ expands value functions that are representable by QMIX. Since individual action-value network and penalty network are universal approximators, $\algoname$ can learn all DEC-POMDP satisfying the assumption (1).

% \note{computational complexity}
% Computational complexity of QMIX and $\algoname$ can be qualitatively compared. Typically, representational complexity and computational complexity are in a trade-off relationship. Comparing QMIX with VDN, representational and computational complexity increase together because summation part of VDN is replaced by monotonic neural network. However, even if $\algoname$ has larger representational complexity than QMIX, computational complexity is not always larger. QMIX constructs that weight of a monotonic neural network through extra state information and another network, hypernetworks. Without weight sharing, computational complexity of hypernetworks increases dramatically as neural networks become deeper. Otherwise, $\algoname$ can use extra state information without using hypernetworks.

% \note{update process}
% Update process proceeds end-to-end to minimize TD-error from centralized action-value function. Like the standard DQN, target network and replay buffer are used, and all networks are trained at once to minimize global loss function. At the end of learning, each agent is controlled decentralized using only its individual action-value function.

% \section{Example: A Matrix Game}

% \begin{table}[!htb]
%     \caption{An example of a cooperative matrix game}
    
%     \begin{subtable}{.48\linewidth}
%       \centering
%         \begin{tabular} { |P{1.3cm}||P{1.3cm}|c|}      \hline
%      $$  & $A$ & $B$ \\      \hline \hline
%      $A$ & $4$ & $2$   \\      \hline
%      $B$ & $2$  & $0$  \\      \hline
%   \end{tabular}
%   \caption{a monotonic payoff matrix}
%   \label {table:monotone}
%     \end{subtable}%
%     \begin{subtable}{.48\linewidth}
%       \centering
%         \begin{tabular} { |P{1.3cm}||P{1.3cm}|c|P{1.3cm}|}      \hline
%      $$  & $A$ & $B$ \\      \hline \hline
%      $A$ & $4$ & $2$   \\      \hline
%      $B$ & $2$  & $3$  \\      \hline
%   \end{tabular}
%   \caption{a non-monotonic payoff matrix}
%   \label {table:non-monotone}
%     \end{subtable} 
%     \label{table:payoff}
% \end{table}

% A matrix game is the simplest form of cooperative multi-agent problem. This game is one-step game which has only one state and two actions per agent. Team reward is determined through a payoff matrix and joint action. 

% The assumptions of VDN (additivity), QMIX (monotonicity) and $\algoname$ ({\bf IGM}) indicate that games like Table~\ref{table:monotone} can be completely represented. In game theoretic view, this game has a unique Nash Equilibrium and can converge to this point as a best response dynamics. On the other hand, games like Table~\ref{table:non-monotone} is theoretically representable by only our $\algoname$. VDN and QMIX can not escape from a local optimal situation with $\bm{u}^{\max} = (B,B)$, but $\algoname$ makes it possible by transforming a game like Table~\ref{table:non-monotone} into a game like Table~\ref{table:monotone} with regularizer $F(\bm{\tau},\bm{u})$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 5.method_backup_dw.tex <==
\section{$\algoname$: Learning to Factorize with Transformation \note{2 page}}

In this section, we propose a new approach called $\algoname$, which
takes advantages of CTDE and factorizes all factorizable tasks.  The
key ideas is to transform the original joint action-value function
$\Qtot$ into a new one $\Qtot'$ that is easily factorizable with the
optimal actions in the original and the transformed joint action-value
functions unchanged. To this end, we estimate $\Qtot'$ as a neural
network which can be decomposed into individual action-value function.

In the following subsections, we first mathematically show that under
what condition $\Qtot$ is factorizable and prove that any factorizable
value function is ensured to be factorized by this transform-based
method.  Next, we present the overall network architecture of
$\algoname$, and details of the network and trainging method follows.

% Now we propose a new approach called $\algoname$, which have advantages of CTDE like VDN and QMIX, but can represent a much richer class of action-value functions with regularization. We additionally make a factorable $\Qtot'$ from original centralized $\Qtot$:
% \begin{align}
% \Qtot'(\bm{\tau},\bm{u}) &= \sum_{i=1}^n Q_i(\tau_i, u_i), \\
% \arg\max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}) &= \arg\max_{\bm{u}} \Qtot'(\bm{\tau},\bm{u}), \label{eq:argmax_cond}
% \end{align}
% where $Q_i(\tau_i, u_i)$ is factorized individual action-value functions from $\Qtot'$. With \ref{eq:argmax_cond}, $\algoname$ allows optimal action selection by greedy decentralized action selection. Key to our method is when the $\Qtot'$ is exist and how to find appropriate $\Qtot'$.

\subsection{Transformation Condition}



% We aim at ensuring the condition, which we call IMC (Individual Max Condition) that a global argmax performed on $\Qtot$ yields
% the same result as a set of individual argmax operations
% performed on each $Q_a$:
We now derive the necessary and sufficient condition of $[Q_i]$ for satisfying {\bf IGM}, which provides a useful guideline on how to factorize the global joint action-value function $\Qtot.$ We first define $\Qtot'$ as: %To this end, we first introduce two functions $Q_i$ and $\Qtot'$, modified ones from $Q_i$ and $\Qtot$. $[Q_i]$ is a some linearly scaled version of the $[Q_i]$, so $\arg\max_{u_i} Q_i(\tau_i, u_i) = \arg\max_{u_i} Q_i(\tau_i, u_i) $ is satisfied. Then, $\Qtot'$ is defined as:
% denote the global and individual value functions as $\Atot(\bm{\tau}) = \Qtot(\bm{\tau},\bm{u}) - \max_{\bm{u}} \Qtot(\bm{\tau},\bm{u})$ and $A_i({\tau_i}) = Q_i({\tau_i},{u_i}) - \max_{{u_i}} Q_i({\tau_i},{u_i}).$ Then, we introduce two functions $Q_i$ and $\Qtot'$, modified ones from $Q_i$ and $\Qtot$, defined as:
\begin{align}
    % Q_i(\tau_i, u_i) & := A_i(\tau_i, u_i), \label{eq:q_prime} \\ 
\Qtot'(\bm{\tau},\bm{u}) & := \sum_{i=1}^n Q_i(\tau_i, u_i). \label{eq:define_qtprime}
\end{align}

% \begin{comment}
% Next, we define the following two variant functions of $Q_i$ and $\Qtot$ as follows: 
% \begin{align}
%     Q_i(\tau_i, u_i) & := Q_i(\tau_i, u_i) - V_i({\tau_i}), \label{eq:q_prime} \\ 
% \Qtot'(\bm{\tau},\bm{u})& := \sum_{i=1}^n Q_i(\tau_i, u_i) 
% \end{align}
% % \begin{align}
% % u^i_{\max} &= \arg\max_{u^{i}}Q_i(\tau^i,u^{i}), \hspace{0.5cm}
% % \Vtot(\bm{\tau}) = \max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}), \hspace{0.5cm} 
% % V_i({\tau^{i}}) = \max_{{u^{i}}} Q_i({\tau^{i}},{u^{i}})
% % \end{align}(3
% % Now, for a given $\alpha >0,$ we define the following two functions:
% Then, by denoting $F(\bm{\tau},\bm{u})$ as
% \begin{align}
% \label{eq:define_F}
% F(\bm{\tau},\bm{u}) &:= \sum_{i=1}^n Q_i(\tau_i, u_i) - ( \Qtot(\bm{\tau},\bm{u}) - \Vtot(\bm{\tau})), 
% \end{align}
% we can rewrite $\Qtot'$ as:
% \begin{align}
% \label{eq:define_qtprime}
% \Qtot^{\prime}(\bm{\tau},\bm{u}) = \Qtot(\bm{\tau},\bm{u}) - \Vtot(\bm{\tau})  + F(\bm{\tau},\bm{u}).
% \end{align}
% % and thus 
% % $\arg\max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}) = \arg\max_{\bm{u}} \Qtot'(\bm{\tau},\bm{u}).$ 
% \end{comment}

% Denote $\bm{\bar{u}} = [u^{\max}_i]_{i=1}^N,$ where 
% $u^{\max}_i = \arg\max_{u^{i}}Q_i(\tau_i,u_i).$ Theorem~\ref{thm:ifonlyif} states the necessary and sufficient condition of a collection of individual value functions $[Q_i]_{i=1}^N$ for the {\bf IGM} condition. 

Let greedy action $\bar{u}_{i} = \arg\max_{u_{i}}Q_i(\tau_i,u_i)$, and a collection of the greedy actions $\bm{\bar{u}} = [\bar{u}_{i}]_{i=1}^N.$% and denote the global advantage functions as $\Atot(\bm{\tau},\bm{u}) = \Qtot(\bm{\tau},\bm{u}) -  \Qtot(\bm{\tau},\bm{\bar{u}})$ 
%and $\Atot'(\bm{\tau},\bm{u}) = \Qtot'(\bm{\tau},\bm{u}) -  \Qtot'(\bm{\tau},\bm{\bar{u}})$, . 
We now present sufficient condition of $\Qtot'$ to satisfy {\bf IGM} condition.

\begin{theorem}
\label{thm:ifonlyif}
For a given global action-value function $\Qtot$ and a collection of individual 
action-value functions $[Q_i]_{i=1}^N,$ if the following condition on $\Qtot'$ is satisfied, then {\bf IGM} condition is also satisfied for the given $\Qtot$ and $[Q_i]$: 
\begin{align}
\label{eq:regular_cond}
\Qtot'(\bm{\tau},\bm{u}) - \Qtot(\bm{\tau},\bm{u}) + \Vtot(\bm{\tau}) &= 
\begin{cases}
    0,& \text{\rm if} \quad \bm{u} = \bm{\bar{u}}\\
    \geq 0,              & \text{\rm otherwise},
\end{cases}
\end{align}
Where $\Vtot(\bm{\tau}) = \Qtot(\bm{\tau},\bm{\bar{u}}) -  \Qtot'(\bm{\tau},\bm{\bar{u}})$.
\end{theorem}


%Let $\Vtot(\bm{\tau}) = \Qtot(\bm{\tau},\bm{\bar{u}}) -  \Qtot'(\bm{\tau},\bm{\bar{u}})$, left-hand side of the equation also can be represented as $\Qtot'(\bm{\tau},\bm{u}) - \Qtot(\bm{\tau},\bm{u}) + \Vtot(\bm{\tau}).$ 
% Where $\Vtot(\bm{\tau}) = \Qtot(\bm{\tau},\bm{\bar{u}}) -  \Qtot'(\bm{\tau},\bm{\bar{u}}).$ The proof is shown in Appendix.


The proof is shown in Appendix. We now present how we use {\bf Theorem~\ref{thm:ifonlyif}} to facilitate the factorization into the each agent's individual local action-value function, which naturally leads to the optimization of the global joint action-value function. Our goal is to find $[Q_i]$ that satisfies {\bf IGM} for a given $\Qtot$. 
It becomes challenging to find such 
$[Q_i]$ unless the underlying game has special properties such as additivity (as in VDN) or monotonicity 
(as in QMIX). Our novel idea is to find $[Q_i]$ satisfying {\bf IGM} indirectly by constructing them so as to meet an alternate condition expressed by \eqref{eq:regular_cond}.%, which turns out to be both necessary and sufficient for {\bf IGM} by {\bf Theorem~\ref{thm:ifonlyif}} and {\bf Theorem~\ref{thm:ifonlyif2}}. 

{\bf Theorem~\ref{thm:ifonlyif}} states that for given $\Qtot$,
$Q_i$ satisfies {\bf IGM}, if it satisfies \eqref{eq:regular_cond}. 
Then, if we construct $[Q_i]$ to meet \eqref{eq:regular_cond}, then those $[Q_i]$ automatically become the individual action-value functions that factorize $\Qtot$.

In addition, we now present \eqref{thm:ifonlyif2} to show necessity of \eqref{eq:regular_cond}, as follows.
\begin{theorem}
\label{thm:ifonlyif2}
For a given global action-value function $\Qtot$ is factorizable, then there always exist action-value functions $[Q_i]_{i=1}^N,$ which satisfies the condition \eqref{eq:regular_cond}.% if the following condition on $\Qtot'$ is satisfied, then {\bf IGM} condition is also satisfied for the given $\Qtot$ and $[Q_i]$: 
\end{theorem}
The proof is shown in Appendix. Necessity in {\bf Theorem~\ref{thm:ifonlyif2}} guarantees that that there always exists 
$[Q_i]$ satisfying \eqref{eq:regular_cond}. So $\algoname$'s representation is always applicable to all factorizable tasks.

Additionally, we now introduce more tight, but still satisfactory condition of the $\Qtot'$.

\begin{corollary}

\label{cor:min}
For a given global action-value function $\Qtot$ and a collection of individual 
action-value functions $[Q_i]_{i=1}^N,$ if there exist $\Qtot'$ which satisfies the condition \eqref{eq:regular_cond}, then there also exist $\Qtot'$ which satisfies \eqref{eq:regular_cond} and the following condition: 
\begin{align}
\label{eq:min_cond}
\min_{u_i}(\Qtot'(\bm{\tau},u_i,\bm{u_{-i}}) - \Qtot(\bm{\tau},u_i,\bm{u_{-i}}) + \Vtot(\bm{\tau})) = 0,
\end{align}
where $\bm{u_{-i}} = \bm{u} \setminus u_i.$
\end{corollary}

If the left-hand side of the equation is greater than zero for given $\tau$ and $\bm{u_{-i}}$, it is easy to find such $\Qtot'$ by parallel translation $Q_i(\tau, u_i)$ without modifying greedy actions. we now present two neural network structures, the one learns to satisfy the condition \eqref{eq:regular_cond} with lower complexity, and the other learns to satisfy the condition \eqref{eq:min_cond} with higher complexity.

% It is easy to find such $Q_i$ if the game has special properties such as additivity of monotonicity. However, it is impossible to find $Q_i$ in general for games that satisfy {\bf IGM} through existing methods. Our novel idea is not to find the $Q_i$ that satisfies {\bf IGM} directly, but to find the $Q_i$ to satisfy the new condition that is equivalent to satisfy the {\bf IGM}.

% Given $\Qtot$ and $Q_i$, the new condition is represented by \eqref{eq:define_F} and \eqref{eq:regular_cond}. The new condition has the same meaning as the existing condition {\bf IGM}, and is easy to handle practically. Theorem~\ref{thm:ifonlyif} tells how the two conditions are connected. The necessary condition of our Theorem~\ref{thm:ifonlyif} is that $\Qtot$ and $Q_i$ satisfy {\bf IGM}, if $\Qtot$ and $Q_i$ satisfy \eqref{eq:regular_cond}. Then, if we make $Q_i$ satisfies \eqref{eq:regular_cond}, then such $Q_i$ automatically becomes a function that factorizes $\Qtot$. Also, sufficient condition proves that there is always $F$ satisfies condition \eqref{eq:define_F}. We will introduce more details about how to use this condition in Section~\ref{sec:method}.

% The meaning of $F$ can be understood through the modified action-value functions $\Qtot'$ and $Q_i$. Given $\Qtot$ and $Q_i$, $\Qtot'$ corresponds to a kind of {\em regularized} global action-value function by taking the summation of $\Qtot$ and $F$ as in \eqref{eq:define_qtprime}.
% By adding $F$ to $\Qtot$, $\Qtot$ is transformed to $\Qtot'$ that is additively decomposed to $[Q_i]$. We note that new action-value functions $\Qtot'$ and $[Q_i]$ have the same optimal solutions as $\Qtot$ and $[Q_i]$, respectively, by \eqref{eq:q_prime},  \eqref{eq:define_qtprime}, and the condition of $F$ in \eqref{eq:regular_cond}. 
% This enables us to easily learn how to factorize $\Qtot$ by changing our angle through a well-constructed regularizer $F.$

% modifying the shape of the existing function $\Qtot$, but the optimal action is maintained.
% In addition, we can confirm that the newly created $\Qtot'$ and $Q_i$ through  have the same optimal as existing $\Qtot$ and $Q_i$ by condition \eqref{eq:regular_cond}. Therefore, $F$ acts as a regularizer, so it is easy to learn 


% For games that satisfy {\bf IGM} conditions, $\Qtot$ is generally not possible to completely factorize with VDN and QMIX. Instead of factorizing this $\Qtot$, we defined a new joint Q-function $\Qtot'$ which is easy to factorize. $\Qtot$ has the same optimal action as $\Qtot$, and it can be represented in the summation of new individual Q-functions $Q_i$. Also, $Q_i$ has the same optimal action as $Q_i$. The necessary condition of Theorem~\ref{thm:ifonlyif} shows that there exists a new $\Qtot'$ and $Q_i$ for all games that satisfy {\bf IGM} condition. The sufficient condition tell us how to find $\Qtot'$, and the condition is given through the form of regularizer $F(\bm{\tau},\bm{u})$.

% \begin{figure*}[ht]
% \begin{subfigure}[t]{.58\textwidth}
%   \includegraphics[width=\linewidth]{figure/qreg_q1}
%   \caption{Individual Action-Value Networks Structure}
%   \label{fig:rnet1}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}[t]{.40\textwidth}
%   \includegraphics[width=\linewidth]{figure/rnn.pdf}
%   \caption{Agent Network Structure}
%   \label{fig:rnn}
% \end{subfigure}\hspace*{\fill}
% \caption{$\algoname$ Architecture}
% \label{fig:NN}
% \end{figure*}


\begin{figure*}[h]
  \centering
 \includegraphics[width=0.92\textwidth]{figure/NN_QREG.pdf}
\caption{$\algoname$ Architecture}
  \label{fig:qreg}
\end{figure*}

\begin{figure*}[h]
  \centering
 \includegraphics[width=0.92\textwidth]{figure/NN_QREG-adv.pdf}
\caption{$\algoname$-adv Architecture}
  \label{fig:qreg-adv}
\end{figure*}

\begin{figure*}[ht]
\begin{subfigure}[t]{.5\textwidth}
  \includegraphics[width=\linewidth]{figure/NN_VDN.pdf}
  \caption{VDN Structure}
  \label{fig:vdn}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}[t]{.5\textwidth}
  \includegraphics[width=\linewidth]{figure/NN_QMIX.pdf}
  \caption{QMIX Structure}
  \label{fig:qmix}
\end{subfigure}\hspace*{\fill}
\caption{VDN and QMIX Architecture}
\label{fig:NN}
\end{figure*}

% \begin{figure*}[h]
%   \centering
%  \includegraphics[width=0.92\textwidth]{figure/QREG}
% \caption{$\algoname$ Architecture}
%   \label{fig:NN}
% \end{figure*}

\subsection{Method}\label{sec:method}

% \begin{figure}
%   \includegraphics[width=1\linewidth]{figure/pqmix_temp.pdf}
%   \caption{Provisional pqmix architecture}
%   \label{fig:pqmix}
% \end{figure}
% \begin{comment}
  

% \begin{figure*}[ht]
% \begin{subfigure}[t]{.32\textwidth}
%   \includegraphics[width=\linewidth]{figure/rnn.pdf}
%   \caption{Individual Action-Value Network}
%   \label{fig:rnn}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}[t]{.27\textwidth}
%   \includegraphics[width=\linewidth]{figure/rnet1.pdf}
%   \caption{Soft Regularization Network}
%   \label{fig:rnet1}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}[t]{.40\textwidth}
%   \includegraphics[width=\linewidth]{figure/rnet2.pdf}
%   \caption{Hard Regularization Network}
%   \label{fig:rnet2}
% \end{subfigure}\hspace*{\fill}
% \caption{$\algoname$ architecture}
% \label{fig:NN2}
% \end{figure*}
% \end{comment}



In this section, we propose a new method of value function factorization, which we call $\algoname$, inspired by our theoretical analysis in {\bf Theorem~\ref{thm:ifonlyif}}.  In centralized Q-learning, we learn $\Qtot$ through function approximators such as neural networks with a centralized trainer. Now we use $Q_i$ as the $Q_i$ in the last section for simplicity. In this paper, we propose $\algoname$ to approximate and factorize $\Qtot$, consisting of three separate estimators: (i) a action-value function for $\Qtot'$, which can be factorized into individual action-value networks $Q_i$, (ii) a value network for $\Vtot$, and (iii) a global action-value network for $\Qtot$. Figure~\ref{fig:NN} shows the overall structure of $\algoname$ and of three estimators inside $\algoname$.
Since we construct loss function to satisfy the condition \eqref{eq:regular_cond} from {\bf Theorem~\ref{thm:ifonlyif}}, $\Qtot'$ can be factorized into individual action-value function $Q_i$ and also satisfy $\arg\max\Qtot' = \arg\max\Qtot.$
This ensures that we train decentralized policies at individual agents in a centralized fashion, which follows the CTDE paradigm.
% We fist present the architecture of $\algoname$ first, followed by that of three estimators. 

We generate three modules of $\algoname$ as follows.
\begin{align*}
&\text{\bf Individual action-value networks} \  f_{\text{q}}: (\tau_i,u_i) \mapsto Q_i, \cr \quad
&\text{\bf Global action-value network} \  f_{\text{r}}: (\bm{\tau}, \bm{u}) \mapsto \Qtot, \cr
  &\text{\hspace{0cm}} \text{\bf Value network} \  f_{\text{v}}: \bm{\tau} \mapsto
    \Vtot. 
\end{align*}

As $\Qtot$ is learned, the estimators are updated through the following condition \eqref{eq:regular_cond}. If $Q_i, \Vtot$, and $\Qtot$ are trained well so as to satisfy the condition in \eqref{eq:regular_cond}, then the learned individual action-value functions are trained to also satisfy {\bf IGM}, thus factorizing $\Qtot$ well. This ensures that we train decentralized policies at individual agents in a centralized fashion. Figure~\ref{fig:NN} shows the overall structure of $\algoname$ and those of three modules inside $\algoname$. The overall architecture is learned through a combination of three modules. And we will introduce each network one by one. Detailed structures are introduced in Appendix.

\paragraph{Individual action-value networks} For each agent, there is an action-value network that takes its own action-observation history $\tau_i$ as input and outputs action-values $Q_i(\tau,\cdot)$ and hidden features of the agent $h_i(\tau,\cdot) = [h_{Q,i}(\tau,\cdot),h_{V,i}(\tau)]$, where $h_{Q,i}(\tau,\cdot)$ is hidden features of the action-values and $h_{V,i}(\tau)$ is hidden features of the values. This action-value network is used for two purposes. From the agents' perspective, each agent can determine its own action by calculating action-value for a given $\tau_i$. From perspective of a centralized trainer, it is also used to calculate $Q_i$ for $\Qtot'$, and $h_i(\tau_i, u_i)$ for input of the global action-value network.  

% \begin{figure}[h!]
%   \centering
%  \includegraphics[width=0.9\columnwidth]{figure/qnet}
% \caption{Action-Value Network}
%   \label{fig:qnet}
% \end{figure}

\paragraph{Global action-value network} We now present the global action-value networks, that is originally from the global action-value function $\Qtot$. Unlike individual action-value networks, which outputs the Q-values for each possible action, Global action-value networks takes the selected action as input and outputs the Q-value of selected action. Instead of directly using the $(\bm{\tau},\bm{u})$ for the input of the global action-value network, we use combined hidden features $\sum_i h_{Q,i}(\tau_i, u_i)$ from the individual action-value networks as input of the global action-value network for efficiency.

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]
    \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$u_1$}{$u_2$}& A & B & C\\ \hline \hline
        A & \textbf{8}& -12 & -12 \\ \hline
        B & -12 & 0 & 0 \\ \hline
        C & -12 & 0 & 0 \\ \hline
        \end{tabular}
        \subcaption{Non-monotonic cooperative matrix game}
        \label{table:p7orig}
    \end{minipage}
    \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$Q_1$}{$Q_2$} & \textbf{4.16}(A) & 2.29(B) & 2.29(C)\\ \hline \hline
        \textbf{3.84}(A) & \textbf{8.00}  & 6.13 & 6.12 \\ \hline
        -2.06(B) & 2.10 & 0.23 & 0.23 \\ \hline
        -2.25(C) & 1.92 & 0.04 & 0.04 \\ \hline
        \end{tabular}
        \subcaption{$Q_1, Q_2,$ and $\Qtot'$ for $\algoname$}
        \label{table:matrix-qreg}
    \end{minipage}\\
    \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$u_1$}{$u_2$}& A & B & C\\ \hline \hline
        A & \textbf{8.00}  & -12.02 & -12.02 \\ \hline
        B & -12.00 & 0.00 & 0.00 \\ \hline
        C & -12.00 & 0.00 & -0.01 \\ \hline
        \end{tabular}
        \subcaption{$\Qtot$ for $\algoname$}
        \label{table:matrix-qreg'}
    \end{minipage}
    \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$u_1$}{$u_2$}& A & B & C\\ \hline \hline
        A & \textbf{0.00}  & 18.14 & 18.14 \\ \hline
        B & 14.11 & 0.23 & 0.23 \\ \hline
        C & 13.93 & 0.05 & 0.05 \\ \hline
        \end{tabular}
        \subcaption{$\Qtot' - \Qtot$ for $\algoname$}
        \label{table:matrix-F}
    \end{minipage}\\
        \begin{minipage}{.48\linewidth}
      \centering
        \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
            \hline
            \backslashbox{$Q_1$}{$Q_2$} & -3.14(A) & \textbf{-2.29}(B) & -2.41(C)\\ \hline \hline
            -2.29(A) & -5.42  & -4.57 & -4.70 \\ \hline
            -1.22(B) & -4.35 & -3.51 & -3.63 \\ \hline
            \textbf{-0.73}(C) & -3.87 & \textbf{-3.02} & -3.14 \\ \hline
        \end{tabular}
        \subcaption{$Q_1, Q_2,$ and $\Qtot$ for VDN}
        \label{table:matrix-vdn}
    \end{minipage}
    \begin{minipage}{.48\linewidth}
      \centering
         \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
        \hline
        \backslashbox{$Q_1$}{$Q_2$} & -0.92(A) & 0.00(B) & \textbf{0.01}(C)\\ \hline \hline
        -1.02(A) & -8.08  & -8.08 & -8.08 \\ \hline
        \textbf{0.11}(B) & -8.08 & 0.01 & \textbf{0.03} \\ \hline
        0.10(C) & -8.08 & 0.01 & 0.02 \\ \hline
        \end{tabular}
        \subcaption{$Q_1, Q_2,$ and $\Qtot$ for QMIX}
        \label{table:matrix-qmix}
    \end{minipage}
        \caption{Payoff matrix of the one-step game and reconstructed $\Qtot$ results on the game. bold means optimal/greedy action/s from the state-action value}
\end{table*}

\paragraph{Value network} Value network is responsible for computing scalar state-value, like $V(s)$ in the dueling network \citep{wang2016dueling}, but our value network is not to learn which states are valuable. The state-value is independent of selected action for a given $\bm{\tau}$. Thus, value network does not contribute to determine action, and is just used to calculate the loss of \eqref{eq:regular_cond}. Like global action-value network, we use combined hidden features $\sum_i h_{V,i}(\tau_i)$ from the individual action-value networks as input of the global action-value network.

\paragraph{Counterfactual global networks}
We now present counterfactual global network to efficiently calculate  $\Qtot(\bm{\tau},\cdot,\bm{u}_{-i})$ and $\Qtot'(\bm{\tau},\cdot,\bm{u}_{-i})$ for all agents with only one forward pass. To this end, instead of using global action-value network, each agent has counterfactual global network and it outputs $\Atot(\bm{\tau},\cdot,\bm{u}_{-i})$ for each possible action for given other agents' action. As global action-value network, we use $h_{V,i}(\tau_i)$ and combined hidden features from other agent $\sum_{j\ne i} h_{Q,j}(\tau_j,u_j).$ Finally, $\Qtot'(\bm{\tau},\cdot,\bm{u}_{-i})$ is calculated by $Q_i(\tau_i,\cdot) + \sum_{j\ne i} Q_j(\tau_j,u_j).$

\paragraph{Loss function of \algoname} We now present the loss function of our algorithms. We use totally 3 loss functions to train the both $\algoname$ and $\algoname$-adv architectures. First loss function is to minimize the squared TD-error, and the others are to satisfy the condition \eqref{eq:regular_cond} or \eqref{eq:min_cond}. During centralized training, we use the algorithm introduced in DQN \citep{mnih2015human} to update networks.
We maintain the target network and replay buffer, which store the sample $(\bm{\tau},\bm{u},r, \bm{\tau}')$, and we update the parameters to minimize the loss function defined as:
\begin{align*} 
L(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&=
\lambda_1 L_1 + \lambda_2 L_2 + \lambda_3 L_3
, \cr \quad
L_{adv}(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&=
\lambda_1 L_1 + \lambda_2 L_2 + \lambda_4 L_4
, \cr \quad
L_1(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&= (\Qtot(\bm{\tau},\bm{u}) - y(r, \bm{\tau}'; \bm{\theta}^{-}))^{2},\cr \quad
L_2(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&= (\Qtot'(\bm{\tau},\bm{\bar{u}}) - \hQtot(\bm{\tau},\bm{\bar{u}}) + \Vtot(\bm{\tau}))^{2}, \cr \quad
L_3(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&= \min(\Qtot'(\bm{\tau},\bm{u}) - \hQtot(\bm{\tau},\bm{u}) + \Vtot(\bm{\tau}),0)^{2}, \cr \quad
L_4(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&= {1 \over n}\sum_i\min_{u_i}D(\bm{\tau},u_i,\bm{u}_{-i}),
\label{eq:lossF} 
\end{align*} 

where $y(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}) = (r + \gamma \Qtot(\bm{\tau}', \bm{u}'^{\max};\theta '))$,  $D(\bm{\tau},u_i,\bm{u}_{-i}) = (\Qtot'(\bm{\tau},u_i,\bm{u}_{-i}) - \hQtot(\bm{\tau},u_i,\bm{u}_{-i}) + + \Vtot(\bm{\tau}))^{2},$ and $\hQtot$ means the parameters of $\Qtot$ is not trained by the loss. $\bm{\theta}^{-}$ are parameters of a target network as in DQN. We set hyperparameters $\lambda_1, \lambda_2, \lambda_3$, and $\lambda_4$ to all 1s. At the end of learning, each agent is controlled in a decentralized fashion using only its own individual action-value function.

% \subsection{Training Regularization Network}\label{sec:regular}

% We now present the regularization network, which is key to our method. In order to successfully factorize $\Qtot$ into individual action-value functions $Q_i$ ({\em i.e.}, $Q_i$ satisfies {\bf IGM}), $F$ should satisfy condition \eqref{eq:regular_cond}. We propose two structures: (i) soft regularization network and (ii) hard regularization network that approximates $F$. 

% \paragraph{Soft regularization network} The soft regularization network has a module, which computes $F(\bm{\tau},\bm{u})$. $F(\bm{\tau},\bm{u})$ is always greater than or equal to 0 by absolute operation. To make regularization network satisfies condition \eqref{eq:regular_cond}, we propose objective can be written as:
% \begin{align*} 
% &L_F(\bm{\tau}, \bm{u}^{\max}; \bm{\theta}):= F(\bm{\tau},\bm{u}^{\max};\theta)^{2}.
% \end{align*}

% The input $\bm{u}^{\max}$ to calculate the loss is from individual action-value functions.  If the loss is zero, we can verify that $F$ equals to 0 when $\bm{u}=\bm{\bar{u}}$. In this way, we can guarantee that condition \eqref{eq:regular_cond} holds.

% % \begin{figure}[h!]
% %   \centering
% %  \includegraphics[width=0.7\columnwidth]{figure/rnet}
% % \caption{Regularization Network}
% %   \label{fig:rnet}
% % \end{figure}

% % We construct the regularization network to output $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{\bar{u}}))^2$.
% % For any function $R$, we can verify that $F(\bm{\tau},\bm{u})$ is always greater than or equal to 0 and that $F$ equals to 0 when $\bm{u}=\bm{\bar{u}}$. In this way, during training $F$, $\Qtot'$, and $\Vtot$, we can always guarantee that condition \eqref{eq:regular_cond} holds.



% % \begin{figure}[h!]
% %   \centering
% %  \includegraphics[width=0.5\columnwidth]{figure/vnet}
% % \caption{Value Network}
% %   \label{fig:vnet}
% % \end{figure}

% During centralized training, we use the algorithm introduced in DQN \citep{mnih2015human} to update networks.
% We maintain the target network and replay buffer, which store the sample $(\bm{\tau},\bm{u},r, \bm{\tau}')$, and we update the parameters to minimize the loss function defined as:
% \begin{align*} 
% L(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&=
% L_Q + \lambda L_F
% , \cr \quad
% L_Q(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}):&= (\Qtot(\bm{\tau},\bm{u};\theta) - y(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}))^{2},\cr \quad
% L_F(\bm{\tau}, \bm{u}^{\max}; \bm{\theta}):&= F(\bm{\tau},\bm{u}^{\max};\theta)^{2},
% \label{eq:lossF} 
% \end{align*} 
% where $y(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}) = (r + \gamma \max_{\bm{u}'} \Qtot(\bm{\tau}', \bm{u}';\theta '))$ and $\lambda$ is hyperparameter. At the end of learning, each agent is controlled in a decentralized fashion using only its own individual action-value function.

% \paragraph{Hard regularization network} Now we present additional method to implement regularization network. The network computes $R(\bm{\tau},\bm{u})$ instead of $F(\bm{\tau},\bm{u})$ by taking $\bm{\tau}, \bm{u}$ as input. For any function $R$, we can confirm $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{u}_{\max}))^2$ is always greater than or equal to 0 , and it is 0 when $\bm{u}=\bm{u}_{\max}$. This is consistent with condition \eqref{eq:regular_cond} of $F$, so we can learn $F(\bm{\tau},\bm{u})$ as we update $R(\bm{\tau},\bm{u}$). 


% \paragraph{Comparison}

% A key feature of the soft regularization network is its smoothness. Soft regularization network is not always satisfied the condition \eqref{eq:regular_cond}, but the network has more representational complexity than hard regularization network and it is differentiable.
% On the contrary, hard regularization network is always satisfied the condition \eqref{eq:regular_cond}, but representational complexity is restricted during training. Also, there is a problem that argmax operation is non differentiable.



\subsection{Matrix game}

To compare the performance of the representational complexity of VDN , QMIX and $\algoname$, we devise a matrix game with two agents. The matrix game is the simplest form of cooperative multi-agent problem. The game is a one-step game with only one state and three actions per agent as shown in Table~\ref{table:p7orig}. The team reward is determined is through a payoff matrix and joint action. We trained VDN, QMIX, and QREG through a full exploration for 20,000 episodes in two matrix games. For simplicity, we delete value network and set value to all 0s. Detailed settings are introduced in Appendix





% \begin{table}[!ht]
% \caption{Non-monotonic cooperative matrix game}
% \label{table:p7orig}
% \vskip 0.15in
% \begin{center}
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         & A & B & C\\ \hline \hline
%         A & \textbf{8}& -12 & -12 \\ \hline
%         B & -12 & 0 & 0 \\ \hline
%         C & -12 & 0 & 0 \\ \hline
%     \end{tabular}
% \end{center}
% \vskip -0.1in
% \end{table}


% \begin{table*}[!ht]
% \caption{Non-monotonic cooperative matrix game}
% \label{table:p7orig2}
% \vskip 0.15in
% \begin{center}
%     \begin{tabular}{|P{1.3cm}||P{1.5cm}|P{1.5cm}|P{1.5cm}|}
%         \hline
%         \backslashbox{$Q_1$}{$Q_2$} & A:-3.14 & B:\textbf{-2.29} & C:-2.41\\ \hline \hline
%         -2.29 & -5.42  & -4.57 & -4.70 \\ \hline
%         -1.22 & -4.35 & -3.51 & -3.63 \\ \hline
%         \textbf{-0.73} & -3.87 & \textbf{-3.02} & -3.14 \\ \hline
%     \end{tabular}
% \subcaption{$Q_1, Q_2,$ and $\Qtot$ for VDN}
% \label{table:matrix-vdn}
%     \begin{tabular}{|P{1.3cm}||P{1.5cm}|P{1.5cm}|P{1.5cm}|}
%         \hline
%         \backslashbox{$Q_1$}{$Q_2$} & -0.92 & 0.00 & \textbf{0.01}\\ \hline \hline
%         -1.02 & -8.08  & -8.08 & -8.08 \\ \hline
%         \textbf{0.11} & -8.08 & 0.01 & \textbf{0.03} \\ \hline
%         0.10 & -8.08 & 0.01 & 0.02 \\ \hline
%     \end{tabular}
% \subcaption{$Q_1, Q_2,$ and $\Qtot$ for QMIX}
% \label{table:matrix-qmix}
% \medskip
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         \backslashbox{$Q_1$}{$Q_2$} & \textbf{4.16} & 2.29 & 2.29\\ \hline \hline
%         \textbf{3.84} & \textbf{8.00}  & 6.13 & 6.12 \\ \hline
%         -2.06 & 2.10 & 0.23 & 0.23 \\ \hline
%         -2.25 & 1.92 & 0.04 & 0.04 \\ \hline
%     \end{tabular}
% \subcaption{$Q_1, Q_2,$ and $\Qtot'$ for $\algoname$}
% \label{table:matrix-qreg}
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         & A & B & C\\ \hline \hline
%         A & \textbf{0.00}  & 18.14 & 18.14 \\ \hline
%         B & 14.11 & 0.23 & 0.23 \\ \hline
%         C & 13.93 & 0.05 & 0.05 \\ \hline
%     \end{tabular}
% \subcaption{$F$ for $\algoname$}
% \label{table:matrix-F}
%     \begin{tabular}{|P{1.3cm}||P{1.3cm}|P{1.3cm}|P{1.3cm}|}
%         \hline
%         & A & B & C\\ \hline \hline
%         A & \textbf{8.00}  & -12.02 & -12.02 \\ \hline
%         B & -12.00 & 0.00 & 0.00 \\ \hline
%         C & -12.00 & 0.00 & -0.01 \\ \hline
%     \end{tabular}
% \subcaption{$\Qtot$ for $\algoname$}
% \label{table:matrix-qreg'}
% \end{center}
% \vskip -0.1in
% \end{table*}



Table~\ref{table:matrix-vdn} and Table~\ref{table:matrix-qmix} illustrate that VDN and QMIX learned the sub-optimal policy. However, our algorithm restored $\Qtot$ accurately and learned $\Qtot'$, which is easy to factorize as shown in Table~\ref{table:matrix-qreg} and Table~\ref{table:matrix-qreg'}.


% \textbf{additional design }

% \textbf{Computational Complexity}
% Computational complexity of QMIX and $\algoname$ can be qualitatively compared. Typically, representational complexity and computational complexity are in a trade-off relationship. Comparing QMIX with VDN, representational and computational complexity increase together because summation part of VDN is replaced by monotonic neural network. However, even if $\algoname$ has larger representational complexity than QMIX, computational complexity is not always larger. QMIX constructs that weight of a monotonic neural network through extra state information and another network, hypernetworks. Without weight sharing, computational complexity of hypernetworks increases dramatically as neural networks become deeper. Otherwise, $\algoname$ can use extra state information without using hypernetworks.

% We now present the regularization network which is a key part of our method. We construct $F$ to satisfy \eqref{eq:regular_cond} and update $Q_i$ and $F$ together. The regularization network computes $R(\bm{\tau},\bm{u})$ instead of $F(\bm{\tau},\bm{u})$ by taking $\bm{\tau}, \bm{u}$ as input, as shown in Figure~\ref{fig:rnet}. For any function $R$, we can confirm $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{u^{\max}}))^2$ is always greater than or equal to 0 and is 0 when $\bm{u}=\bm{u^{\max}}$. This is consistent with condition \eqref{eq:regular_cond} of $F$, so we can learn $F(\bm{\tau},\bm{u})$ as we update $R(\bm{\tau},\bm{u}$). 

% Instead of  doing this, we can consider other method that update $Q_i$ by designing loss function to satisfy \eqref{eq:regular_cond}. The advantage of this method is that the relationship between $F$ and $Q_i$ becomes clear because $F$ is expressed through $Q_i$ without using independent networks for $F$. Also, the amount of computation can be reduced because no additional networks are used. However, we already have a loss functions to learn $\Qtot$, so it is difficult to balance two loss functions at the same time. Therefore, we designed the regularization network using the previous method. 


% \begin{comment}
%   In this section, we propose a new method of value function factorization, which we call $\algoname$, inspired by our theoretical analysis in Theorem~\ref{thm:ifonlyif}.
% In the centralized Q-learning, we learn $\Qtot$ through function approximators such as  neural networks with a centralized trainer. We learn $\Qtot'$ so as to be factorized and also to satisfy $\arg\max\Qtot' = \arg\max\Qtot.$ Our network includes three separate estimators: (i) individual action-value networks for $Q_1, Q_2, ... Q_n$, (ii) value network for $\Vtot$, and (iii) regularization network for $F$. As $\Qtot$ is learned, the estimators are updated through the following equation $\Qtot = \Vtot + \Qtot' - F(\bm{\tau},\bm{u})$. If $Q_i, \Vtot$, and $F$ are trained well so as to satisfy the condition in \eqref{eq:regular_cond}, then the learned individual action-value functions are trained to also satisfy {\bf IGM}, thus factorizing $\Qtot$ well. This ensures that we train decentralized policies at individual agents in a centralized fashion. Figure~\ref{fig:NN} shows the overall structure of $\algoname$ and those of three modules inside $\algoname$. $\Qtot$ is learned through a combination of three modules, as depicted in Figure~\ref{fig:qgnet}. And we will introduce each network one by one.


% \subsection{Centralized training with decentralized execution}
% We consider a centralized training with decentralized execution, where the learning algorithm has access to all local action-observation histories $\bm{\tau}$ in conjunction with the global state $\bm{s}$, but each agent's learned policy can condition only on its own action-observation history $\tau_i$.

% Update process proceeds end-to-end to minimize TD-error from centralized action-value function. Like the standard DQN, target network and replay buffer are used, and all networks are trained at once to minimize global loss function. At the end of learning, each agent is controlled decentralized using only its individual action-value function.

% \subsection{Regularization network} 

% First, regularization network is a key part of our method. We construct $F$ to satisfy \eqref{eq:regular_cond} and update $Q_i$ and $F$ together. The regularization network computes $R(\bm{\tau},\bm{u})$ instead of $F(\bm{\tau},\bm{u})$ by taking $\bm{\tau}, \bm{u}$ as input, as shown in Figure~\ref{fig:rnet}. For any function $R$, we can confirm $F(\bm{\tau},\bm{u}) = (R(\bm{\tau},\bm{u}) - R(\bm{\tau},\bm{\bar{u}}))^2$ is always greater than or equal to 0 and is 0 when $\bm{u}=\bm{\bar{u}}$. This is consistent with condition \eqref{eq:regular_cond} of $F$, so we can learn $F(\bm{\tau},\bm{u})$ as we update $R(\bm{\tau},\bm{u}$). 

% Instead of  doing this, we can consider other method that update $Q_i$ by designing loss function to satisfy \eqref{eq:regular_cond}. The advantage of this method is that the relationship between $F$ and $Q_i$ becomes clear because $F$ is expressed through $Q_i$ without using independent networks for $F$. Also, the amount of computation can be reduced because no additional networks are used. However, we already have a loss functions to learn $\Qtot$, so it is difficult to balance two loss functions at the same time. Therefore, we designed the regularization network using the previous method. 


% \subsection{Individual action-value and value networks} Figure~\ref{fig:qnet} illustrates structure of individual action-value networks. For each agent, there is an action-value network that takes its own action-observation history $\tau^i$ as input and outputs action-values $Q_i$. This action-value network is used for two purposes. From the agents' perspective, each agent can determine its own action by calculating action-value for a given $\tau^i$. From perspective of a centralized trainer, it is also used to calculate $\Qtot'$, one of modules that form $\Qtot$.
% Finally, value network is responsible for computing scalar state-value as illustrated in Figure~\ref{fig:vnet} like $V(s)$ in the dueling network \citep{wang2016dueling}. The state-value is independent of selected action for a given $\bm{\tau}$. Thus, value network does not contribute to determine action, and is just used to calculate $\Qtot$.

% \end{comment}



% \note{overall view}
% This section introduces general framework of $\algoname$ architecture. The neural network architecture we propose is decomposed into individual action-value networks and penalty networks. Figure shows the overall settings. Individual action-value networks are used to select action for each agent. Given action-observation histories of each agents, individual action-value networks compute action-value function. 

% \note{penalty network explanation}
% Penalty networks is the key part of our method. Penalty network takes as state and set of actions, and generates penalty value. Penalty term is determined by difference between two outputs of the penalty network. One output is for the selected action and the other is for the argmax action. So, if every agent chooses its argmax action, then two outputs are same and penalty term becomes zero. In this case, Centralized action-value function is decomposed into summation of individual action-value functions. On the other hand, if some agents select different actions, then penalty term is greater than zero. Thus, we can see that when each agent selects its argmax action, the centralized action-value function is maximized.

% \note{representational complexity or expressive power}
% Expressive power of our neural network architecture can be confirmed as follows. Intuitively, if the output of the penalty network is always 0, our network is the same as VDN. Moreover, $\algoname$ expands value functions that are representable by QMIX. Since individual action-value network and penalty network are universal approximators, $\algoname$ can learn all DEC-POMDP satisfying the assumption (1).

% \note{computational complexity}
% Computational complexity of QMIX and $\algoname$ can be qualitatively compared. Typically, representational complexity and computational complexity are in a trade-off relationship. Comparing QMIX with VDN, representational and computational complexity increase together because summation part of VDN is replaced by monotonic neural network. However, even if $\algoname$ has larger representational complexity than QMIX, computational complexity is not always larger. QMIX constructs that weight of a monotonic neural network through extra state information and another network, hypernetworks. Without weight sharing, computational complexity of hypernetworks increases dramatically as neural networks become deeper. Otherwise, $\algoname$ can use extra state information without using hypernetworks.

% \note{update process}
% Update process proceeds end-to-end to minimize TD-error from centralized action-value function. Like the standard DQN, target network and replay buffer are used, and all networks are trained at once to minimize global loss function. At the end of learning, each agent is controlled decentralized using only its individual action-value function.

% \section{Example: A Matrix Game}

% \begin{table}[!htb]
%     \caption{An example of a cooperative matrix game}
    
%     \begin{subtable}{.48\linewidth}
%       \centering
%         \begin{tabular} { |P{1.3cm}||P{1.3cm}|c|}      \hline
%      $$  & $A$ & $B$ \\      \hline \hline
%      $A$ & $4$ & $2$   \\      \hline
%      $B$ & $2$  & $0$  \\      \hline
%   \end{tabular}
%   \caption{a monotonic payoff matrix}
%   \label {table:monotone}
%     \end{subtable}%
%     \begin{subtable}{.48\linewidth}
%       \centering
%         \begin{tabular} { |P{1.3cm}||P{1.3cm}|c|P{1.3cm}|}      \hline
%      $$  & $A$ & $B$ \\      \hline \hline
%      $A$ & $4$ & $2$   \\      \hline
%      $B$ & $2$  & $3$  \\      \hline
%   \end{tabular}
%   \caption{a non-monotonic payoff matrix}
%   \label {table:non-monotone}
%     \end{subtable} 
%     \label{table:payoff}
% \end{table}

% A matrix game is the simplest form of cooperative multi-agent problem. This game is one-step game which has only one state and two actions per agent. Team reward is determined through a payoff matrix and joint action. 

% The assumptions of VDN (additivity), QMIX (monotonicity) and $\algoname$ ({\bf IGM}) indicate that games like Table~\ref{table:monotone} can be completely represented. In game theoretic view, this game has a unique Nash Equilibrium and can converge to this point as a best response dynamics. On the other hand, games like Table~\ref{table:non-monotone} is theoretically representable by only our $\algoname$. VDN and QMIX can not escape from a local optimal situation with $\bm{\bar{u}} = (B,B)$, but $\algoname$ makes it possible by transforming a game like Table~\ref{table:non-monotone} into a game like Table~\ref{table:monotone} with regularizer $F(\bm{\tau},\bm{u})$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

